DataPilot: Utilizing Quality and Usage Information for Subset Selection during Visual Data Preparation

Selecting relevant data subsets from large, unfamiliar datasets can be difficult. We address this challenge by modeling and visualizing two kinds of auxiliary information: (1) quality - the validity and appropriateness of data required to perform certain analytical tasks; and (2) usage - the historical utilization characteristics of data across multiple users. Through a design study with 14 data workers, we integrate this information into a visual data preparation and analysis tool, DataPilot. DataPilot presents visual cues about "the good, the bad, and the ugly" aspects of data and provides graphical user interface controls as interaction affordances, guiding users to perform subset selection. Through a study with 36 participants, we investigate how DataPilot helps users navigate a large, unfamiliar tabular dataset, prepare a relevant subset, and build a visualization dashboard. We find that users selected smaller, effective subsets with higher quality and usage, and with greater success and confidence.

==> commands.tex <==
\newcommand{\bpstart}[1]{
\noindent{\textbf{#1}}%
}

\newcommand{\todo}[1]{\textcolor{red}{[TODO: #1]}}

\newcommand{\highlight}[1]{\textcolor{green}{#1}}

\newcommand{\app}{\mbox{DataPilot}\xspace}

\newcommand{\paragraphHeadingSpace}{\vspace{4px}}

% Control (reduce) the spacing between a float(ed) figure and the text
\setlength{\textfloatsep}{4pt}
\setlength{\dbltextfloatsep}{4pt}

% Participant Identities
% First-choice but 'Q' as a sub/super script takes up more than 1 line apparently -- not good.
% \newcommand{\pc}[1]{$P_{#1}^{C}$}
% \newcommand{\pq}[1]{$P_{#1}^{Q}$}
% \newcommand{\pe}[1]{$P_{#1}^{E}$}


\newcommand{\pc}[1]{$B_{#1}$}
\newcommand{\pq}[1]{$Q_{#1}$}
\newcommand{\pe}[1]{$D_{#1}$}
\newcommand{\pde}[1]{$E_{#1}$}
\newcommand{\ses}[1]{$S_{#1}$}

% Custom Colors
\definecolor{D}{HTML}{00856b} % 00b894
\definecolor{Q}{HTML}{6c5ce7}
\definecolor{B}{HTML}{e17055}
\definecolor{DE}{HTML}{4834d4}
\definecolor{red}{HTML}{ff0000}
\definecolor{linkcolor}{HTML}{647382}
\definecolor{citecolor}{HTML}{647382} %
\definecolor{urlcolor}{rgb}{0.4,0.2,0.2}
\definecolor{sqlcolor}{HTML}{965d67}
\definecolor{smtcolor}{HTML}{5d968c}
\definecolor{commentcolor}{HTML}{4B0082}
\definecolor{high}{HTML}{2ecc71}
\definecolor{medium}{HTML}{f1c40f}
\definecolor{low}{HTML}{e74c3c}
\definecolor{unchecked}{HTML}{efefef}
\definecolor{cellhighlight}{HTML}{cefaee}


% Collaborator Comments
\newcommand{\arpit}[1]{\textcolor{red}{[Arpit: #1]}}
\newcommand{\alex}[1]{\textcolor{brown}{#1}}
\newcommand{\ryan}[1]{\textcolor{blue}{[Ryan: #1]}}
\newcommand{\atanu}[1]{\textcolor{blue}{#1}}
\newcommand{\eunyee}[1]{\textcolor{red}{#1}}
\newcommand{\fan}[1]{\textcolor{red}{[Fan: #1]}}
\newcommand{\jane}[1]{\textcolor{teal}{\textbf{[Jane: #1]}}}
\newcommand{\janeText}[1]{\textcolor{teal}{#1}}
\newcommand{\shunan}[1]{\textcolor{yellow}{#1}}

% NEW COLOR DEFINITIONS FOR THE REVISE AND RESUBMIT PLAN
\definecolor{darkgreen}{HTML}{009432}
\definecolor{darkblue}{HTML}{2980b9}
\definecolor{darkred}{HTML}{c0392b}

% Strikethroughs are causing general issues; we will only go with text in red, no strikethroughs.
% \newcommand{\cut}[1]{\textcolor{darkred}{\st{#1}}}

% Use this for ANNOTATED VERSION
% \newcommand{\cut}[1]{\textcolor{darkred}{#1}} % REMOVE without strikethrough
% \newcommand{\edit}[1]{\textcolor{darkblue}{#1}} % REVISE / EDIT
% \newcommand{\add}[1]{\textcolor{darkgreen}{#1}} % ADD new content

%  Use this for UNANNOTATED VERSION
\newcommand{\cut}[1]{}
\newcommand{\edit}[1]{#1}
\newcommand{\add}[1]{#1}

==> packages.tex <==
\usepackage{soul}
\usepackage{enumitem}
\usepackage{tabularx}
\usepackage{multirow}
\usepackage{color}
\usepackage{xcolor}
\usepackage{xspace}
\usepackage{subfig}
\usepackage{graphicx}
\usepackage{listings}
\usepackage{fontawesome}

\makeatletter
\newcommand{\xslalph}[1]{\expandafter\@xslalph\csname c@#1\endcsname}
\newcommand{\@xslalph}[1]{%
    \ifcase#1\or B\or Q\or D%
    \else\@ctrerr\fi%
}

\lstdefinestyle{SQLStyle}{
language=SQL,
basicstyle=\footnotesize, 
mathescape,
keywordstyle=\color{sqlcolor}\bfseries,
commentstyle=\color{commentcolor}\ttfamily,
deletekeywords ={Role,ROLE},
literate = {-}{-}1, % <------ trick!
}
